Optimizing a-DCF for Spoofing-Robust Speaker Verification

Automatic speaker verification (ASV) systems are vulnerable to spoofing attacks. We propose a spoofing-robust ASV system optimized directly for the recently introduced architecture-agnostic detection cost function (a-DCF), which allows targeting a desired trade-off between the contradicting aims of user convenience and robustness to spoofing. We combine a-DCF and binary cross-entropy (BCE) with a novel straightforward threshold optimization technique. Our results with an embedding fusion system on ASVspoof2019 data demonstrate relative improvement of $13\%$ over a system trained using BCE only (from minimum a-DCF of $0.1445$ to $0.1254$). Using an alternative non-linear score fusion approach provides relative improvement of $43\%$ (from minimum a-DCF of $0.0508$ to $0.0289$).

==> original_intro.tex <==
\section{Introduction}

Automatic Speaker Verification (ASV) systems verify that a given speech utterance corresponds to a claimed identity \cite{reynolds94_asriv}. Like many ML models, ASV systems are susceptible to such adversarial inputs, prompting attackers to produce similar attempts at deceiving the ASV system when they submit audio samples for verification. This is known as a replay attack \cite{kinnunen2017} if the attacker resubmits a copy of the target’s legitimate recording, and a synthesis attack \cite{todisco2019asvspoof} if the submission is generated from scratch using speech synthesis, also known as text-to-speech (TTS) systems. To counter these risks, spoofing countermeasure (CM) systems have been developed that attempt to catch such spoofed audio and, when paired with an ASV system, substantially increase its tolerance to spoofing attempts \cite{todisco2019asvspoof}. For many years, the scientific study of such spoofing countermeasures was conducted independently from ASV; both types of systems were usually considered in isolation, with no attempt to study the combined impact of both types of systems. However, with recent advances, spoofing-robust speaker verification systems, which function more or less like regular systems of ASV, while being made far more tolerant to spoofing, are finally becoming attainable.

Since a spoofing detector is like a speaker detector, it can be evaluated with the same binary metrics described above. When these two systems work together, there are three input classes: target, non-target, and spoof, and simultaneous evaluation of a complete tandem system of the speaker and spoof detector calls for another metric that captures this fact. The tandem detection cost function (t-DCF) \cite{kinnunen2020tandem} was developed for this purpose, and it can be used to evaluate any spoofing-robust two-class ASV (speaker verification) system. Note that a binary metric must be complemented by a binary reference set, meaning that the t-DCF requires two separate speaker/nonspeaker and spoof/nonspoof labels, and it’s hard to produce such labels blindly for new unlabelled speech data. Because of the binary-class need in each reference dataset, the t-DCF can not be used to evaluate alternative approaches with only a single score. In response, \cite{shim2024adcf} proposed a novel metric derived from the old DCF metric and named it the \emph{architecture agnostic detection cost function} (a-DCF). The name architecture agnostic is used in contrast with the t-DCF which is only meaningful with a tandem system, where speaker and spoofing detection subsystems are performed separately and in a cascaded sequential way. Notice that there can be many ways of combining speaker and spoofing detection; for example, they can be closely coupled and jointly optimized, or even we can have speaker and spoofing detection almost done independently leaving little to gain by combining. The only requirement of the architecture-agnostic detection cost function (a-DCF) is that the system must produce a single score indicating if the input utterance likely possesses a claimed identity and is likely genuine.

Despite many studies evaluating systems using this tandem metric, the original ASV and CM systems are not trained to minimize the a-DCF. Instead, they are trained using their respective loss functions for their individual tasks, without considering the presence of the other system. Since the a-DCF metric relies on hard counts of misses and false accepts, it is a non-differentiable metric that cannot be directly optimized using gradient descent methods. However, metrics can be "softened" (made differentiable) by approximating the non-differentiable operations with differentiable ones. We adopt this technique to extend a soft (differentiable) version of the detection cost function (DCF) metric \cite{mingote19_interspeech} to accommodate a-DCF.

In this work, we make the following contributions:

\begin{itemize}
    \item We propose a differentiable approximation of the a-DCF metric, termed soft a-DCF, enabling its integration into the training process of machine learning models.
    \item We provide a theoretical analysis and empirical validation of the proposed soft a-DCF metric, demonstrating its effectiveness and robustness in various speaker verification and spoofing detection scenarios.
    \item We conduct extensive experiments comparing the performance of models trained with soft a-DCF against those trained with traditional loss functions.
\end{itemize}

By integrating a differentiable version of the a-DCF into model training, we aim to enhance the performance and robustness of speaker verification systems against spoofing attacks, ultimately contributing to the advancement of secure and reliable biometric authentication technologies.
